Pipe Routing with Topology Control for UAV Networks

Routing protocols help in transmitting the sensed data from UAVs monitoring the targets (called target UAVs) to the BS. However, the highly dynamic nature of an autonomous, decentralized UAV network leads to frequent route breaks or traffic disruptions. Traditional routing schemes cannot quickly adapt to dynamic UAV networks and/or incur large control overhead and delays. To establish stable, high-quality routes from target UAVs to the BS, we design a hybrid reactive routing scheme called pipe routing that is mobility, congestion, and energy-aware. The pipe routing scheme discovers routes on-demand and proactively switches to alternate high-quality routes within a limited region around the active routes (called the pipe) when needed, reducing the number of route breaks and increasing data throughput. We then design a novel topology control-based pipe routing scheme to maintain robust connectivity in the pipe region around the active routes, leading to improved route stability and increased throughput with minimal impact on the coverage performance of the UAV network.

==> Tables/1T-30.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1
\begin{adjustbox}{width=\textwidth}
 
\begin{tabular}{|cc|c!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccccc|}

\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{\textbf{30 UAVs}}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\% Node\\ Failure\end{tabular}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}2 km, 2 km{]}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}4 km, 4 km{]}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}1.5 km, 5 km{]}}} \\ \cline{4-18} 
\multicolumn{2}{|c|}{} &
   &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} \\ \hline
\multicolumn{1}{|c|}{\multirow{12}{*}{\textbf{20 m/s}}} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Route\\ Up \%\end{tabular}}} &
  \textbf{0} &
  \multicolumn{1}{c|}{97} &
  \multicolumn{1}{c|}{91} &
  \multicolumn{1}{c|}{84} &
  \multicolumn{1}{c|}{78} &
  100 &
  \multicolumn{1}{c|}{82} &
  \multicolumn{1}{c|}{66} &
  \multicolumn{1}{c|}{59} &
  \multicolumn{1}{c|}{41} &
  98 &
  \multicolumn{1}{c|}{48} &
  \multicolumn{1}{c|}{30} &
  \multicolumn{1}{c|}{26} &
  \multicolumn{1}{c|}{21} &
  94 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{86} &
  \multicolumn{1}{c|}{81} &
  \multicolumn{1}{c|}{73} &
  100 &
  \multicolumn{1}{c|}{72} &
  \multicolumn{1}{c|}{52} &
  \multicolumn{1}{c|}{46} &
  \multicolumn{1}{c|}{34} &
  98 &
  \multicolumn{1}{c|}{23} &
  \multicolumn{1}{c|}{24} &
  \multicolumn{1}{c|}{21} &
  \multicolumn{1}{c|}{16} &
  87 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{84} &
  \multicolumn{1}{c|}{79} &
  \multicolumn{1}{c|}{70} &
  100 &
  \multicolumn{1}{c|}{61} &
  \multicolumn{1}{c|}{47} &
  \multicolumn{1}{c|}{43} &
  \multicolumn{1}{c|}{31} &
  95 &
  \multicolumn{1}{c|}{30} &
  \multicolumn{1}{c|}{20} &
  \multicolumn{1}{c|}{18} &
  \multicolumn{1}{c|}{11} &
  92 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Route\\ Breaks\end{tabular}}} &
  \textbf{0} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{18} &
  \multicolumn{1}{c|}{142} &
  \multicolumn{1}{c|}{24} &
  0 &
  \multicolumn{1}{c|}{21} &
  \multicolumn{1}{c|}{30} &
  \multicolumn{1}{c|}{187} &
  \multicolumn{1}{c|}{30} &
  0 &
  \multicolumn{1}{c|}{21} &
  \multicolumn{1}{c|}{18} &
  \multicolumn{1}{c|}{102} &
  \multicolumn{1}{c|}{23} &
  0 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{14} &
  \multicolumn{1}{c|}{19} &
  \multicolumn{1}{c|}{132} &
  \multicolumn{1}{c|}{30} &
  1 &
  \multicolumn{1}{c|}{26} &
  \multicolumn{1}{c|}{30} &
  \multicolumn{1}{c|}{139} &
  \multicolumn{1}{c|}{34} &
  2 &
  \multicolumn{1}{c|}{16} &
  \multicolumn{1}{c|}{20} &
  \multicolumn{1}{c|}{78} &
  \multicolumn{1}{c|}{20} &
  2 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{17} &
  \multicolumn{1}{c|}{24} &
  \multicolumn{1}{c|}{123} &
  \multicolumn{1}{c|}{30} &
  1 &
  \multicolumn{1}{c|}{32} &
  \multicolumn{1}{c|}{33} &
  \multicolumn{1}{c|}{131} &
  \multicolumn{1}{c|}{29} &
  3 &
  \multicolumn{1}{c|}{20} &
  \multicolumn{1}{c|}{20} &
  \multicolumn{1}{c|}{65} &
  \multicolumn{1}{c|}{14} &
  3 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
  \multirow{3}{*}{\textbf{Fairness}} &
  \textbf{0} &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.69} &
  \multicolumn{1}{c|}{0.69} &
  \multicolumn{1}{c|}{0.7} &
  0.69 &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.71} &
  \multicolumn{1}{c|}{0.71} &
  \multicolumn{1}{c|}{0.70} &
  0.68 &
  \multicolumn{1}{c|}{0.67} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.69} &
  0.68 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{0.61} &
  \multicolumn{1}{c|}{0.67} &
  \multicolumn{1}{c|}{0.67} &
  \multicolumn{1}{c|}{0.68} &
  0.66 &
  \multicolumn{1}{c|}{0.62} &
  \multicolumn{1}{c|}{0.68} &
  \multicolumn{1}{c|}{0.68} &
  \multicolumn{1}{c|}{0.67} &
  0.65 &
  \multicolumn{1}{c|}{0.65} &
  \multicolumn{1}{c|}{0.68} &
  \multicolumn{1}{c|}{0.68} &
  \multicolumn{1}{c|}{0.66} &
  0.62 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{0.6} &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.66} &
  0.65 &
  \multicolumn{1}{c|}{0.64} &
  \multicolumn{1}{c|}{0.65} &
  \multicolumn{1}{c|}{0.65} &
  \multicolumn{1}{c|}{0.66} &
  0.58 &
  \multicolumn{1}{c|}{0.63} &
  \multicolumn{1}{c|}{0.69} &
  \multicolumn{1}{c|}{0.69} &
  \multicolumn{1}{c|}{0.66} &
  0.59 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Visitation\\ Frequency\end{tabular}}} &
  \textbf{0} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  4 &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  3 &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  3 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  3 &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  3 &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  2 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  3 &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  2 &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  2 \\ \hline
\Xhline{1pt}
\multicolumn{1}{|c|}{\multirow{12}{*}{\textbf{40 m/s}}} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Route\\ Up \%\end{tabular}}} &
  \textbf{0} &
  \multicolumn{1}{c|}{96} &
  \multicolumn{1}{c|}{88} &
  \multicolumn{1}{c|}{77} &
  \multicolumn{1}{c|}{76} &
  100 &
  \multicolumn{1}{c|}{77} &
  \multicolumn{1}{c|}{57} &
  \multicolumn{1}{c|}{45} &
  \multicolumn{1}{c|}{42} &
  99 &
  \multicolumn{1}{c|}{39} &
  \multicolumn{1}{c|}{26} &
  \multicolumn{1}{c|}{20} &
  \multicolumn{1}{c|}{19} &
  94 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{85} &
  \multicolumn{1}{c|}{75} &
  \multicolumn{1}{c|}{72} &
  99 &
  \multicolumn{1}{c|}{66} &
  \multicolumn{1}{c|}{48} &
  \multicolumn{1}{c|}{38} &
  \multicolumn{1}{c|}{32} &
  98 &
  \multicolumn{1}{c|}{23} &
  \multicolumn{1}{c|}{15} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{13} &
  93 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{93} &
  \multicolumn{1}{c|}{83} &
  \multicolumn{1}{c|}{73} &
  \multicolumn{1}{c|}{68} &
  100 &
  \multicolumn{1}{c|}{60} &
  \multicolumn{1}{c|}{40} &
  \multicolumn{1}{c|}{33} &
  \multicolumn{1}{c|}{27} &
  98 &
  \multicolumn{1}{c|}{26} &
  \multicolumn{1}{c|}{14} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{11} &
  93 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Route\\ Breaks\end{tabular}}} &
  \textbf{0} &
  \multicolumn{1}{c|}{20} &
  \multicolumn{1}{c|}{39} &
  \multicolumn{1}{c|}{267} &
  \multicolumn{1}{c|}{42} &
  0 &
  \multicolumn{1}{c|}{43} &
  \multicolumn{1}{c|}{63} &
  \multicolumn{1}{c|}{314} &
  \multicolumn{1}{c|}{51} &
  0 &
  \multicolumn{1}{c|}{37} &
  \multicolumn{1}{c|}{40} &
  \multicolumn{1}{c|}{169} &
  \multicolumn{1}{c|}{32} &
  0 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{29} &
  \multicolumn{1}{c|}{46} &
  \multicolumn{1}{c|}{249} &
  \multicolumn{1}{c|}{44} &
  1 &
  \multicolumn{1}{c|}{59} &
  \multicolumn{1}{c|}{60} &
  \multicolumn{1}{c|}{248} &
  \multicolumn{1}{c|}{47} &
  2 &
  \multicolumn{1}{c|}{32} &
  \multicolumn{1}{c|}{27} &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{24} &
  2 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{30} &
  \multicolumn{1}{c|}{50} &
  \multicolumn{1}{c|}{241} &
  \multicolumn{1}{c|}{47} &
  1 &
  \multicolumn{1}{c|}{63} &
  \multicolumn{1}{c|}{65} &
  \multicolumn{1}{c|}{221} &
  \multicolumn{1}{c|}{44} &
  3 &
  \multicolumn{1}{c|}{38} &
  \multicolumn{1}{c|}{32} &
  \multicolumn{1}{c|}{88} &
  \multicolumn{1}{c|}{22} &
  3 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
  \multirow{3}{*}{\textbf{Fairness}} &
  \textbf{0} &
  \multicolumn{1}{c|}{0.7} &
  \multicolumn{1}{c|}{0.76} &
  \multicolumn{1}{c|}{0.76} &
  \multicolumn{1}{c|}{0.77} &
  0.77 &
  \multicolumn{1}{c|}{0.70} &
  \multicolumn{1}{c|}{0.76} &
  \multicolumn{1}{c|}{0.76} &
  \multicolumn{1}{c|}{0.77} &
  0.73 &
  \multicolumn{1}{c|}{0.75} &
  \multicolumn{1}{c|}{0.77} &
  \multicolumn{1}{c|}{0.77} &
  \multicolumn{1}{c|}{0.77} &
  0.74 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{0.67} &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.75} &
  0.73 &
  \multicolumn{1}{c|}{0.67} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.76} &
  0.71 &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.74} &
  \multicolumn{1}{c|}{0.74} &
  \multicolumn{1}{c|}{0.76} &
  0.68 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{0.64} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.74} &
  0.73 &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.74} &
  0.69 &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.74} &
  0.68 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Visitation\\ Frequency\end{tabular}}} &
  \textbf{0} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{6} &
  7 &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{6} &
  6 &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{6} &
  6 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  6 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  5 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  5 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  6 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  5 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  4 \\ \hline
\Xhline{1pt}   
\end{tabular}

\end{adjustbox}
\end{table*}

==> Tables/1T-50.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1
\begin{adjustbox}{width=\textwidth}
 
\begin{tabular}{|cc|c!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccccc|}

\hline
\multicolumn{2}{|c|}{\multirow{2}{*}{\textbf{50 UAVs}}} &
  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\% Node\\ Failure\end{tabular}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}2 km, 2 km{]}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}4 km, 4 km{]}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}1.5 km, 5 km{]}}} \\ \cline{4-18} 
\multicolumn{2}{|c|}{} &
   &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} \\ \hline
\multicolumn{1}{|c|}{\multirow{12}{*}{\textbf{20 m/s}}} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Route\\ Up \%\end{tabular}}} &
  \textbf{0} &
  \multicolumn{1}{c|}{99} &
  \multicolumn{1}{c|}{98} &
  \multicolumn{1}{c|}{90} &
  \multicolumn{1}{c|}{90} &
  100 &
  \multicolumn{1}{c|}{97} &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{80} &
  \multicolumn{1}{c|}{78} &
  100 &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{87} &
  \multicolumn{1}{c|}{71} &
  \multicolumn{1}{c|}{67} &
  100 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{98} &
  \multicolumn{1}{c|}{96} &
  \multicolumn{1}{c|}{89} &
  \multicolumn{1}{c|}{86} &
  100 &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{90} &
  \multicolumn{1}{c|}{78} &
  \multicolumn{1}{c|}{69} &
  99 &
  \multicolumn{1}{c|}{91} &
  \multicolumn{1}{c|}{76} &
  \multicolumn{1}{c|}{63} &
  \multicolumn{1}{c|}{54} &
  99 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{97} &
  \multicolumn{1}{c|}{96} &
  \multicolumn{1}{c|}{89} &
  \multicolumn{1}{c|}{81} &
  100 &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{88} &
  \multicolumn{1}{c|}{76} &
  \multicolumn{1}{c|}{60} &
  100 &
  \multicolumn{1}{c|}{85} &
  \multicolumn{1}{c|}{68} &
  \multicolumn{1}{c|}{57} &
  \multicolumn{1}{c|}{49} &
  99 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Route\\ Breaks\end{tabular}}} &
  \textbf{0} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{166} &
  \multicolumn{1}{c|}{23} &
  0 &
  \multicolumn{1}{c|}{15} &
  \multicolumn{1}{c|}{30} &
  \multicolumn{1}{c|}{315} &
  \multicolumn{1}{c|}{45} &
  0 &
  \multicolumn{1}{c|}{22} &
  \multicolumn{1}{c|}{40} &
  \multicolumn{1}{c|}{355} &
  \multicolumn{1}{c|}{52} &
  0 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{16} &
  \multicolumn{1}{c|}{159} &
  \multicolumn{1}{c|}{30} &
  1 &
  \multicolumn{1}{c|}{27} &
  \multicolumn{1}{c|}{41} &
  \multicolumn{1}{c|}{294} &
  \multicolumn{1}{c|}{51} &
  2 &
  \multicolumn{1}{c|}{37} &
  \multicolumn{1}{c|}{50} &
  \multicolumn{1}{c|}{305} &
  \multicolumn{1}{c|}{57} &
  2 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{21} &
  \multicolumn{1}{c|}{160} &
  \multicolumn{1}{c|}{29} &
  2 &
  \multicolumn{1}{c|}{32} &
  \multicolumn{1}{c|}{48} &
  \multicolumn{1}{c|}{289} &
  \multicolumn{1}{c|}{54} &
  2 &
  \multicolumn{1}{c|}{46} &
  \multicolumn{1}{c|}{56} &
  \multicolumn{1}{c|}{269} &
  \multicolumn{1}{c|}{56} &
  3 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
  \multirow{3}{*}{\textbf{Fairness}} &
  \textbf{0} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.85} &
  0.87 &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.85} &
  0.86 &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.85} &
  0.83 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.84} &
  0.85 &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.83} &
  0.82 &
  \multicolumn{1}{c|}{0.83} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.83} &
  0.80 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{0.83} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.83} &
  0.83 &
  \multicolumn{1}{c|}{0.81} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.83} &
  0.80 &
  \multicolumn{1}{c|}{0.82} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.82} &
  0.77 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
  \multirow{3}{*}{\textbf{$V_f$}} &
  \textbf{0} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  6 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  6 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  5 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{5} &
  6 &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{5} &
  5 &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{5} &
  5 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{4} &
  5 &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{4} &
  5 &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{4} &
  4 \\ \hline
\Xhline{1pt} 
\multicolumn{1}{|c|}{\multirow{12}{*}{\textbf{40 m/s}}} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Route\\ Up \%\end{tabular}}} &
  \textbf{0} &
  \multicolumn{1}{c|}{99} &
  \multicolumn{1}{c|}{97} &
  \multicolumn{1}{c|}{82} &
  \multicolumn{1}{c|}{89} &
  100 &
  \multicolumn{1}{c|}{97} &
  \multicolumn{1}{c|}{92} &
  \multicolumn{1}{c|}{66} &
  \multicolumn{1}{c|}{79} &
  100 &
  \multicolumn{1}{c|}{93} &
  \multicolumn{1}{c|}{83} &
  \multicolumn{1}{c|}{56} &
  \multicolumn{1}{c|}{64} &
  100 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{98} &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{81} &
  \multicolumn{1}{c|}{84} &
  100 &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{86} &
  \multicolumn{1}{c|}{63} &
  \multicolumn{1}{c|}{66} &
  100 &
  \multicolumn{1}{c|}{86} &
  \multicolumn{1}{c|}{68} &
  \multicolumn{1}{c|}{48} &
  \multicolumn{1}{c|}{50} &
  100 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{98} &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{81} &
  \multicolumn{1}{c|}{79} &
  100 &
  \multicolumn{1}{c|}{93} &
  \multicolumn{1}{c|}{84} &
  \multicolumn{1}{c|}{63} &
  \multicolumn{1}{c|}{61} &
  100 &
  \multicolumn{1}{c|}{81} &
  \multicolumn{1}{c|}{61} &
  \multicolumn{1}{c|}{43} &
  \multicolumn{1}{c|}{41} &
  100 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
  \multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Route\\ Breaks\end{tabular}}} &
  \textbf{0} &
  \multicolumn{1}{c|}{14} &
  \multicolumn{1}{c|}{29} &
  \multicolumn{1}{c|}{319} &
  \multicolumn{1}{c|}{39} &
  0 &
  \multicolumn{1}{c|}{31} &
  \multicolumn{1}{c|}{66} &
  \multicolumn{1}{c|}{581} &
  \multicolumn{1}{c|}{80} &
  0 &
  \multicolumn{1}{c|}{49} &
  \multicolumn{1}{c|}{85} &
  \multicolumn{1}{c|}{617} &
  \multicolumn{1}{c|}{88} &
  0 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{22} &
  \multicolumn{1}{c|}{39} &
  \multicolumn{1}{c|}{313} &
  \multicolumn{1}{c|}{49} &
  1 &
  \multicolumn{1}{c|}{48} &
  \multicolumn{1}{c|}{91} &
  \multicolumn{1}{c|}{544} &
  \multicolumn{1}{c|}{86} &
  3 &
  \multicolumn{1}{c|}{77} &
  \multicolumn{1}{c|}{107} &
  \multicolumn{1}{c|}{521} &
  \multicolumn{1}{c|}{91} &
  2 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{23} &
  \multicolumn{1}{c|}{45} &
  \multicolumn{1}{c|}{308} &
  \multicolumn{1}{c|}{52} &
  2 &
  \multicolumn{1}{c|}{60} &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{522} &
  \multicolumn{1}{c|}{91} &
  3 &
  \multicolumn{1}{c|}{85} &
  \multicolumn{1}{c|}{107} &
  \multicolumn{1}{c|}{462} &
  \multicolumn{1}{c|}{90} &
  3 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
  \multirow{3}{*}{\textbf{Fairness}} &
  \textbf{0} &
  \multicolumn{1}{c|}{0.91} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.90} &
  0.92 &
  \multicolumn{1}{c|}{0.90} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.90} &
  0.90 &
  \multicolumn{1}{c|}{0.90} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.90} &
  0.88 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.89} &
  0.89 &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.88} &
  0.87 &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.89} &
  0.86 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.88} &
  0.88 &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.88} &
  0.85 &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.88} &
  0.84 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
  \multirow{3}{*}{\textbf{$V_f$}} &
  \textbf{0} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{10} &
  13 &
  \multicolumn{1}{c|}{14} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{10} &
  11 &
  \multicolumn{1}{c|}{14} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{10} &
  11 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{9} &
  11 &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{9} &
  10 &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{9} &
  9 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{30} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{9} &
  11 &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{9} &
  9 &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{9} &
  8 \\ \hline
\Xhline{1pt}   
\end{tabular}

\end{adjustbox}
\end{table*}

==> Tables/table-1target-30UAVs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1
\begin{adjustbox}{width=\textwidth}
 
\begin{tabular}{|cc|c!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccccc|}

\hline
\multicolumn{2}{|c|}{} &
   &
  \multicolumn{5}{c|}{\textbf{Location={[}2000 m, 2000 m{]}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}4000 m, 4000 m{]}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}1500 m, 5000 m{]}}} \\ \cline{4-18} 
\multicolumn{2}{|c|}{\multirow{-2}{*}{\textbf{30 UAVs}}} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\% Node\\ Failure\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} \\ \hline
\Xhline{1pt}   
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{97} &
  \multicolumn{1}{c|}{89} &
  \multicolumn{1}{c|}{83} &
  \multicolumn{1}{c|}{78} &
  100 &
  \multicolumn{1}{c|}{82} &
  \multicolumn{1}{c|}{60} &
  \multicolumn{1}{c|}{56} &
  \multicolumn{1}{c|}{41} &
  98 &
  \multicolumn{1}{c|}{48} &
  \multicolumn{1}{c|}{34} &
  \multicolumn{1}{c|}{23} &
  \multicolumn{1}{c|}{21} &
  94 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{88} &
  \multicolumn{1}{c|}{{\color[HTML]{FF0000} 84}} &
  \multicolumn{1}{c|}{73} &
  100 &
  \multicolumn{1}{c|}{72} &
  \multicolumn{1}{c|}{51} &
  \multicolumn{1}{c|}{46} &
  \multicolumn{1}{c|}{34} &
  98 &
  \multicolumn{1}{c|}{23} &
  \multicolumn{1}{c|}{21} &
  \multicolumn{1}{c|}{21} &
  \multicolumn{1}{c|}{16} &
  87 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Route\\ Up \%\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{93} &
  \multicolumn{1}{c|}{84} &
  \multicolumn{1}{c|}{78} &
  \multicolumn{1}{c|}{68} &
  99 &
  \multicolumn{1}{c|}{60} &
  \multicolumn{1}{c|}{39} &
  \multicolumn{1}{c|}{40} &
  \multicolumn{1}{c|}{24} &
  96 &
  \multicolumn{1}{c|}{17} &
  \multicolumn{1}{c|}{19} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{10} &
  82 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{16} &
  \multicolumn{1}{c|}{140} &
  \multicolumn{1}{c|}{24} &
  0 &
  \multicolumn{1}{c|}{21} &
  \multicolumn{1}{c|}{25} &
  \multicolumn{1}{c|}{185} &
  \multicolumn{1}{c|}{30} &
  0 &
  \multicolumn{1}{c|}{21} &
  \multicolumn{1}{c|}{21} &
  \multicolumn{1}{c|}{91} &
  \multicolumn{1}{c|}{23} &
  0 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{14} &
  \multicolumn{1}{c|}{20} &
  \multicolumn{1}{c|}{131} &
  \multicolumn{1}{c|}{30} &
  1 &
  \multicolumn{1}{c|}{26} &
  \multicolumn{1}{c|}{27} &
  \multicolumn{1}{c|}{139} &
  \multicolumn{1}{c|}{34} &
  2 &
  \multicolumn{1}{c|}{16} &
  \multicolumn{1}{c|}{19} &
  \multicolumn{1}{c|}{77} &
  \multicolumn{1}{c|}{20} &
  2 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Route\\ Breaks\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{18} &
  \multicolumn{1}{c|}{23} &
  \multicolumn{1}{c|}{119} &
  \multicolumn{1}{c|}{32} &
  2 &
  \multicolumn{1}{c|}{34} &
  \multicolumn{1}{c|}{29} &
  \multicolumn{1}{c|}{118} &
  \multicolumn{1}{c|}{25} &
  3 &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{17} &
  \multicolumn{1}{c|}{40} &
  \multicolumn{1}{c|}{14} &
  3 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.71} &
  \multicolumn{1}{c|}{0.70} &
  \multicolumn{1}{c|}{0.70} &
  0.69 &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.69} &
  \multicolumn{1}{c|}{0.70} &
  \multicolumn{1}{c|}{0.70} &
  0.68 &
  \multicolumn{1}{c|}{0.67} &
  \multicolumn{1}{c|}{0.70} &
  \multicolumn{1}{c|}{0.69} &
  \multicolumn{1}{c|}{0.69} &
  0.68 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{0.61} &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.65} &
  \multicolumn{1}{c|}{0.68} &
  0.66 &
  \multicolumn{1}{c|}{0.62} &
  \multicolumn{1}{c|}{0.67} &
  \multicolumn{1}{c|}{0.69} &
  \multicolumn{1}{c|}{0.67} &
  0.65 &
  \multicolumn{1}{c|}{0.65} &
  \multicolumn{1}{c|}{0.69} &
  \multicolumn{1}{c|}{0.69} &
  \multicolumn{1}{c|}{0.66} &
  0.62 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{Fairness}} &
  \textbf{40} &
  \multicolumn{1}{c|}{0.58} &
  \multicolumn{1}{c|}{0.62} &
  \multicolumn{1}{c|}{0.64} &
  \multicolumn{1}{c|}{0.66} &
  0.63 &
  \multicolumn{1}{c|}{0.60} &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.64} &
  \multicolumn{1}{c|}{0.63} &
  0.61 &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.65} &
  \multicolumn{1}{c|}{0.65} &
  \multicolumn{1}{c|}{0.64} &
  0.58 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  4 &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  3 &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  3 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{10} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  3 &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  3 &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  2 \\ \cline{3-18} 
\multicolumn{1}{|c|}{\multirow{-12}{*}{\textbf{20 m/s}}} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Visitation\\ Frequency\end{tabular}}} &
  \textbf{30} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  3 &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  2 &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{2} &
  2 \\ \hline
\Xhline{1pt}   
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{96} &
  \multicolumn{1}{c|}{89} &
  \multicolumn{1}{c|}{78} &
  \multicolumn{1}{c|}{76} &
  100 &
  \multicolumn{1}{c|}{77} &
  \multicolumn{1}{c|}{58} &
  \multicolumn{1}{c|}{41} &
  \multicolumn{1}{c|}{42} &
  99 &
  \multicolumn{1}{c|}{39} &
  \multicolumn{1}{c|}{25} &
  \multicolumn{1}{c|}{18} &
  \multicolumn{1}{c|}{19} &
  94 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{85} &
  \multicolumn{1}{c|}{75} &
  \multicolumn{1}{c|}{72} &
  99 &
  \multicolumn{1}{c|}{66} &
  \multicolumn{1}{c|}{47} &
  \multicolumn{1}{c|}{37} &
  \multicolumn{1}{c|}{32} &
  98 &
  \multicolumn{1}{c|}{23} &
  \multicolumn{1}{c|}{15} &
  \multicolumn{1}{c|}{14} &
  \multicolumn{1}{c|}{13} &
  93 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Route\\ Up \%\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{90} &
  \multicolumn{1}{c|}{78} &
  \multicolumn{1}{c|}{71} &
  \multicolumn{1}{c|}{64} &
  99 &
  \multicolumn{1}{c|}{55} &
  \multicolumn{1}{c|}{33} &
  \multicolumn{1}{c|}{30} &
  \multicolumn{1}{c|}{25} &
  97 &
  \multicolumn{1}{c|}{17} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{9} &
  91 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{20} &
  \multicolumn{1}{c|}{34} &
  \multicolumn{1}{c|}{270} &
  \multicolumn{1}{c|}{42} &
  0 &
  \multicolumn{1}{c|}{43} &
  \multicolumn{1}{c|}{52} &
  \multicolumn{1}{c|}{287} &
  \multicolumn{1}{c|}{51} &
  0 &
  \multicolumn{1}{c|}{37} &
  \multicolumn{1}{c|}{30} &
  \multicolumn{1}{c|}{148} &
  \multicolumn{1}{c|}{32} &
  0 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{29} &
  \multicolumn{1}{c|}{42} &
  \multicolumn{1}{c|}{251} &
  \multicolumn{1}{c|}{44} &
  1 &
  \multicolumn{1}{c|}{59} &
  \multicolumn{1}{c|}{56} &
  \multicolumn{1}{c|}{245} &
  \multicolumn{1}{c|}{47} &
  2 &
  \multicolumn{1}{c|}{32} &
  \multicolumn{1}{c|}{27} &
  \multicolumn{1}{c|}{110} &
  \multicolumn{1}{c|}{24} &
  2 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Route\\ Breaks\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{36} &
  \multicolumn{1}{c|}{49} &
  \multicolumn{1}{c|}{227} &
  \multicolumn{1}{c|}{48} &
  2 &
  \multicolumn{1}{c|}{60} &
  \multicolumn{1}{c|}{51} &
  \multicolumn{1}{c|}{191} &
  \multicolumn{1}{c|}{44} &
  4 &
  \multicolumn{1}{c|}{30} &
  \multicolumn{1}{c|}{25} &
  \multicolumn{1}{c|}{64} &
  \multicolumn{1}{c|}{21} &
  4 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{0.70} &
  \multicolumn{1}{c|}{0.75} &
  \multicolumn{1}{c|}{0.74} &
  \multicolumn{1}{c|}{0.77} &
  0.77 &
  \multicolumn{1}{c|}{0.70} &
  \multicolumn{1}{c|}{0.75} &
  \multicolumn{1}{c|}{0.77} &
  \multicolumn{1}{c|}{0.77} &
  0.73 &
  \multicolumn{1}{c|}{0.75} &
  \multicolumn{1}{c|}{0.76} &
  \multicolumn{1}{c|}{0.77} &
  \multicolumn{1}{c|}{0.77} &
  0.74 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{0.67} &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.75} &
  0.73 &
  \multicolumn{1}{c|}{0.67} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.74} &
  \multicolumn{1}{c|}{0.76} &
  0.71 &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.75} &
  \multicolumn{1}{c|}{0.76} &
  \multicolumn{1}{c|}{0.76} &
  0.68 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{Fairness}} &
  \textbf{40} &
  \multicolumn{1}{c|}{0.64} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.70} &
  \multicolumn{1}{c|}{0.74} &
  0.70 &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.74} &
  0.66 &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.73} &
  0.62 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{6} &
  7 &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{6} &
  6 &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{6} &
  6 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  6 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  5 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  5 \\ \cline{3-18} 
\multicolumn{1}{|c|}{\multirow{-12}{*}{\textbf{40 m/s}}} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Visitation\\ Frequency\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{5} &
  5 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  4 &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{5} &
  4 \\ \hline

\Xhline{1pt}   
\end{tabular}

\end{adjustbox}
\end{table*}

==> Tables/table-1target-50UAVs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1
\begin{adjustbox}{width=\textwidth}
 
\begin{tabular}{|cc|c!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccccc|}

\hline
\multicolumn{2}{|c|}{} &
   &
  \multicolumn{5}{c|}{\textbf{Location={[}2000 m, 2000 m{]}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}4000 m, 4000 m{]}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}1500 m, 5000 m{]}}} \\ \cline{4-18} 
\multicolumn{2}{|c|}{\multirow{-2}{*}{\textbf{50 UAVs}}} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\% Node\\ Failure\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} \\ \hline
\Xhline{1pt}  
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{99} &
  \multicolumn{1}{c|}{97} &
  \multicolumn{1}{c|}{90} &
  \multicolumn{1}{c|}{90} &
  100 &
  \multicolumn{1}{c|}{97} &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{80} &
  \multicolumn{1}{c|}{78} &
  100 &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{85} &
  \multicolumn{1}{c|}{70} &
  \multicolumn{1}{c|}{67} &
  100 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{98} &
  \multicolumn{1}{c|}{96} &
  \multicolumn{1}{c|}{88} &
  \multicolumn{1}{c|}{86} &
  100 &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{90} &
  \multicolumn{1}{c|}{77} &
  \multicolumn{1}{c|}{69} &
  99 &
  \multicolumn{1}{c|}{91} &
  \multicolumn{1}{c|}{78} &
  \multicolumn{1}{c|}{64} &
  \multicolumn{1}{c|}{54} &
  99 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Route\\ Up \%\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{97} &
  \multicolumn{1}{c|}{93} &
  \multicolumn{1}{c|}{89} &
  \multicolumn{1}{c|}{77} &
  100 &
  \multicolumn{1}{c|}{90} &
  \multicolumn{1}{c|}{82} &
  \multicolumn{1}{c|}{72} &
  \multicolumn{1}{c|}{54} &
  100 &
  \multicolumn{1}{c|}{79} &
  \multicolumn{1}{c|}{60} &
  \multicolumn{1}{c|}{51} &
  \multicolumn{1}{c|}{39} &
  99 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{167} &
  \multicolumn{1}{c|}{23} &
  0 &
  \multicolumn{1}{c|}{15} &
  \multicolumn{1}{c|}{29} &
  \multicolumn{1}{c|}{316} &
  \multicolumn{1}{c|}{45} &
  0 &
  \multicolumn{1}{c|}{22} &
  \multicolumn{1}{c|}{37} &
  \multicolumn{1}{c|}{363} &
  \multicolumn{1}{c|}{52} &
  0 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{17} &
  \multicolumn{1}{c|}{168} &
  \multicolumn{1}{c|}{30} &
  1 &
  \multicolumn{1}{c|}{27} &
  \multicolumn{1}{c|}{38} &
  \multicolumn{1}{c|}{300} &
  \multicolumn{1}{c|}{51} &
  2 &
  \multicolumn{1}{c|}{37} &
  \multicolumn{1}{c|}{49} &
  \multicolumn{1}{c|}{308} &
  \multicolumn{1}{c|}{57} &
  2 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Route\\ Breaks\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{15} &
  \multicolumn{1}{c|}{23} &
  \multicolumn{1}{c|}{153} &
  \multicolumn{1}{c|}{32} &
  2 &
  \multicolumn{1}{c|}{36} &
  \multicolumn{1}{c|}{51} &
  \multicolumn{1}{c|}{270} &
  \multicolumn{1}{c|}{50} &
  3 &
  \multicolumn{1}{c|}{50} &
  \multicolumn{1}{c|}{54} &
  \multicolumn{1}{c|}{238} &
  \multicolumn{1}{c|}{50} &
  4 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.85} &
  0.87 &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.85} &
  0.86 &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.85} &
  0.83 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.84} &
  0.85 &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.83} &
  0.82 &
  \multicolumn{1}{c|}{0.83} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.86} &
  \multicolumn{1}{c|}{0.83} &
  0.80 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{Fairness}} &
  \textbf{40} &
  \multicolumn{1}{c|}{0.79} &
  \multicolumn{1}{c|}{0.82} &
  \multicolumn{1}{c|}{0.82} &
  \multicolumn{1}{c|}{0.82} &
  0.81 &
  \multicolumn{1}{c|}{0.79} &
  \multicolumn{1}{c|}{0.82} &
  \multicolumn{1}{c|}{0.81} &
  \multicolumn{1}{c|}{0.81} &
  0.79 &
  \multicolumn{1}{c|}{0.79} &
  \multicolumn{1}{c|}{0.82} &
  \multicolumn{1}{c|}{0.81} &
  \multicolumn{1}{c|}{0.82} &
  0.76 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  6 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  6 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  5 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{10} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{5} &
  6 &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{5} &
  5 &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{5} &
  5 \\ \cline{3-18} 
\multicolumn{1}{|c|}{\multirow{-12}{*}{\textbf{20 m/s}}} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Visitation\\ Frequency\end{tabular}}} &
  \textbf{30} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{4} &
  5 &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{4} &
  4 &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{4} &
  4 \\ \hline
\Xhline{1pt}
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{99} &
  \multicolumn{1}{c|}{97} &
  \multicolumn{1}{c|}{82} &
  \multicolumn{1}{c|}{89} &
  100 &
  \multicolumn{1}{c|}{97} &
  \multicolumn{1}{c|}{92} &
  \multicolumn{1}{c|}{66} &
  \multicolumn{1}{c|}{79} &
  100 &
  \multicolumn{1}{c|}{93} &
  \multicolumn{1}{c|}{82} &
  \multicolumn{1}{c|}{56} &
  \multicolumn{1}{c|}{64} &
  100 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{98} &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{81} &
  \multicolumn{1}{c|}{84} &
  100 &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{87} &
  \multicolumn{1}{c|}{64} &
  \multicolumn{1}{c|}{66} &
  100 &
  \multicolumn{1}{c|}{86} &
  \multicolumn{1}{c|}{69} &
  \multicolumn{1}{c|}{51} &
  \multicolumn{1}{c|}{50} &
  100 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Route\\ Up \%\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{97} &
  \multicolumn{1}{c|}{93} &
  \multicolumn{1}{c|}{80} &
  \multicolumn{1}{c|}{76} &
  100 &
  \multicolumn{1}{c|}{90} &
  \multicolumn{1}{c|}{77} &
  \multicolumn{1}{c|}{58} &
  \multicolumn{1}{c|}{51} &
  99 &
  \multicolumn{1}{c|}{73} &
  \multicolumn{1}{c|}{54} &
  \multicolumn{1}{c|}{39} &
  \multicolumn{1}{c|}{35} &
  99 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{14} &
  \multicolumn{1}{c|}{24} &
  \multicolumn{1}{c|}{321} &
  \multicolumn{1}{c|}{39} &
  0 &
  \multicolumn{1}{c|}{31} &
  \multicolumn{1}{c|}{58} &
  \multicolumn{1}{c|}{580} &
  \multicolumn{1}{c|}{80} &
  0 &
  \multicolumn{1}{c|}{49} &
  \multicolumn{1}{c|}{75} &
  \multicolumn{1}{c|}{629} &
  \multicolumn{1}{c|}{88} &
  1 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{22} &
  \multicolumn{1}{c|}{34} &
  \multicolumn{1}{c|}{321} &
  \multicolumn{1}{c|}{49} &
  1 &
  \multicolumn{1}{c|}{48} &
  \multicolumn{1}{c|}{82} &
  \multicolumn{1}{c|}{547} &
  \multicolumn{1}{c|}{86} &
  3 &
  \multicolumn{1}{c|}{77} &
  \multicolumn{1}{c|}{93} &
  \multicolumn{1}{c|}{550} &
  \multicolumn{1}{c|}{91} &
  2 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Route\\ Breaks\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{31} &
  \multicolumn{1}{c|}{49} &
  \multicolumn{1}{c|}{304} &
  \multicolumn{1}{c|}{54} &
  1 &
  \multicolumn{1}{c|}{70} &
  \multicolumn{1}{c|}{99} &
  \multicolumn{1}{c|}{473} &
  \multicolumn{1}{c|}{91} &
  4 &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{96} &
  \multicolumn{1}{c|}{395} &
  \multicolumn{1}{c|}{80} &
  5 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{0.91} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.90} &
  0.92 &
  \multicolumn{1}{c|}{0.90} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.90} &
  0.90 &
  \multicolumn{1}{c|}{0.90} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.90} &
  0.88 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.89} &
  0.89 &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.88} &
  0.87 &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.89} &
  0.86 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{Fairness}} &
  \textbf{40} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.86} &
  \multicolumn{1}{c|}{0.86} &
  \multicolumn{1}{c|}{0.87} &
  0.86 &
  \multicolumn{1}{c|}{0.82} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.86} &
  \multicolumn{1}{c|}{0.87} &
  0.84 &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.86} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.87} &
  0.83 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{10} &
  13 &
  \multicolumn{1}{c|}{14} &
  \multicolumn{1}{c|}{14} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{10} &
  11 &
  \multicolumn{1}{c|}{14} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{10} &
  11 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{9} &
  11 &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{9} &
  10 &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{9} &
  9 \\ \cline{3-18} 
\multicolumn{1}{|c|}{\multirow{-12}{*}{\textbf{40 m/s}}} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Visitation\\ Frequency\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{8} &
  10 &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{8} &
  8 &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{8} &
  7 \\ \hline
  
\Xhline{1pt}   
\end{tabular}

\end{adjustbox}
\end{table*}

==> Tables/table-3targets-30UAVs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1
\begin{adjustbox}{width=\textwidth}
 
\begin{tabular}{|cc|c!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccccc|}

\hline
\multicolumn{2}{|c|}{} &
   &
  \multicolumn{5}{c|}{\textbf{Location={[}Case 7{]}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}Case5{]}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}Case6{]}}} \\ \cline{4-18} 
\multicolumn{2}{|c|}{\multirow{-2}{*}{\textbf{30 UAVs}}} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\% Node\\ Failure\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} \\ \hline
\Xhline{1pt}
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{93} &
  \multicolumn{1}{c|}{84} &
  \multicolumn{1}{c|}{79} &
  \multicolumn{1}{c|}{72} &
  100 &
  \multicolumn{1}{c|}{68} &
  \multicolumn{1}{c|}{51} &
  \multicolumn{1}{c|}{45} &
  \multicolumn{1}{c|}{39} &
  97 &
  \multicolumn{1}{c|}{39} &
  \multicolumn{1}{c|}{27} &
  \multicolumn{1}{c|}{25} &
  \multicolumn{1}{c|}{18} &
  94 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{91} &
  \multicolumn{1}{c|}{78} &
  \multicolumn{1}{c|}{75} &
  \multicolumn{1}{c|}{65} &
  100 &
  \multicolumn{1}{c|}{53} &
  \multicolumn{1}{c|}{45} &
  \multicolumn{1}{c|}{35} &
  \multicolumn{1}{c|}{33} &
  95 &
  \multicolumn{1}{c|}{37} &
  \multicolumn{1}{c|}{16} &
  \multicolumn{1}{c|}{15} &
  \multicolumn{1}{c|}{16} &
  83 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Route\\ Up \%\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{88} &
  \multicolumn{1}{c|}{75} &
  \multicolumn{1}{c|}{71} &
  \multicolumn{1}{c|}{58} &
  99 &
  \multicolumn{1}{c|}{48} &
  \multicolumn{1}{c|}{35} &
  \multicolumn{1}{c|}{36} &
  \multicolumn{1}{c|}{27} &
  87 &
  \multicolumn{1}{c|}{19} &
  \multicolumn{1}{c|}{15} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{9} &
  78 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{38} &
  \multicolumn{1}{c|}{59} &
  \multicolumn{1}{c|}{426} &
  \multicolumn{1}{c|}{74} &
  0 &
  \multicolumn{1}{c|}{53} &
  \multicolumn{1}{c|}{58} &
  \multicolumn{1}{c|}{349} &
  \multicolumn{1}{c|}{70} &
  0 &
  \multicolumn{1}{c|}{53} &
  \multicolumn{1}{c|}{49} &
  \multicolumn{1}{c|}{286} &
  \multicolumn{1}{c|}{53} &
  1 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{53} &
  \multicolumn{1}{c|}{68} &
  \multicolumn{1}{c|}{389} &
  \multicolumn{1}{c|}{83} &
  2 &
  \multicolumn{1}{c|}{59} &
  \multicolumn{1}{c|}{60} &
  \multicolumn{1}{c|}{259} &
  \multicolumn{1}{c|}{67} &
  4 &
  \multicolumn{1}{c|}{72} &
  \multicolumn{1}{c|}{46} &
  \multicolumn{1}{c|}{159} &
  \multicolumn{1}{c|}{52} &
  4 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Route\\ Breaks\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{67} &
  \multicolumn{1}{c|}{81} &
  \multicolumn{1}{c|}{341} &
  \multicolumn{1}{c|}{77} &
  5 &
  \multicolumn{1}{c|}{67} &
  \multicolumn{1}{c|}{60} &
  \multicolumn{1}{c|}{248} &
  \multicolumn{1}{c|}{56} &
  7 &
  \multicolumn{1}{c|}{57} &
  \multicolumn{1}{c|}{47} &
  \multicolumn{1}{c|}{140} &
  \multicolumn{1}{c|}{35} &
  10 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{0.60} &
  \multicolumn{1}{c|}{0.67} &
  \multicolumn{1}{c|}{0.65} &
  \multicolumn{1}{c|}{0.68} &
  0.60 &
  \multicolumn{1}{c|}{0.65} &
  \multicolumn{1}{c|}{0.71} &
  \multicolumn{1}{c|}{0.69} &
  \multicolumn{1}{c|}{0.68} &
  0.59 &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.71} &
  \multicolumn{1}{c|}{0.69} &
  \multicolumn{1}{c|}{0.67} &
  0.54 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{0.55} &
  \multicolumn{1}{c|}{0.64} &
  \multicolumn{1}{c|}{0.62} &
  \multicolumn{1}{c|}{0.65} &
  0.56 &
  \multicolumn{1}{c|}{0.60} &
  \multicolumn{1}{c|}{0.65} &
  \multicolumn{1}{c|}{0.70} &
  \multicolumn{1}{c|}{0.64} &
  0.49 &
  \multicolumn{1}{c|}{0.63} &
  \multicolumn{1}{c|}{0.67} &
  \multicolumn{1}{c|}{0.68} &
  \multicolumn{1}{c|}{0.65} &
  0.57 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{Fairness}} &
  \textbf{40} &
  \multicolumn{1}{c|}{0.51} &
  \multicolumn{1}{c|}{0.60} &
  \multicolumn{1}{c|}{0.60} &
  \multicolumn{1}{c|}{0.62} &
  0.54 &
  \multicolumn{1}{c|}{0.56} &
  \multicolumn{1}{c|}{0.63} &
  \multicolumn{1}{c|}{0.63} &
  \multicolumn{1}{c|}{0.63} &
  0.48 &
  \multicolumn{1}{c|}{0.59} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.64} &
  0.46 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  3 &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  2 &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  2 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{10} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  2 &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  1 &
  \multicolumn{1}{c|}{4} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  2 \\ \cline{3-18} 
\multicolumn{1}{|c|}{\multirow{-12}{*}{\textbf{20 m/s}}} &
  \multirow{-3}{*}{\textbf{$V_f$}} &
  \textbf{30} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{2} &
  2 &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{2} &
  1 &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{3} &
  \multicolumn{1}{c|}{2} &
  1 \\ \hline
\Xhline{1pt}
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{84} &
  \multicolumn{1}{c|}{72} &
  \multicolumn{1}{c|}{68} &
  100 &
  \multicolumn{1}{c|}{56} &
  \multicolumn{1}{c|}{46} &
  \multicolumn{1}{c|}{38} &
  \multicolumn{1}{c|}{37} &
  96 &
  \multicolumn{1}{c|}{34} &
  \multicolumn{1}{c|}{23} &
  \multicolumn{1}{c|}{19} &
  \multicolumn{1}{c|}{18} &
  96 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{90} &
  \multicolumn{1}{c|}{77} &
  \multicolumn{1}{c|}{67} &
  \multicolumn{1}{c|}{63} &
  100 &
  \multicolumn{1}{c|}{50} &
  \multicolumn{1}{c|}{40} &
  \multicolumn{1}{c|}{33} &
  \multicolumn{1}{c|}{31} &
  96 &
  \multicolumn{1}{c|}{24} &
  \multicolumn{1}{c|}{16} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{11} &
  91 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Route\\ Up \%\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{86} &
  \multicolumn{1}{c|}{70} &
  \multicolumn{1}{c|}{63} &
  \multicolumn{1}{c|}{55} &
  99 &
  \multicolumn{1}{c|}{44} &
  \multicolumn{1}{c|}{35} &
  \multicolumn{1}{c|}{30} &
  \multicolumn{1}{c|}{26} &
  91 &
  \multicolumn{1}{c|}{17} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{9} &
  \multicolumn{1}{c|}{9} &
  86 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{81} &
  \multicolumn{1}{c|}{124} &
  \multicolumn{1}{c|}{796} &
  \multicolumn{1}{c|}{127} &
  0 &
  \multicolumn{1}{c|}{86} &
  \multicolumn{1}{c|}{112} &
  \multicolumn{1}{c|}{610} &
  \multicolumn{1}{c|}{109} &
  1 &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{89} &
  \multicolumn{1}{c|}{440} &
  \multicolumn{1}{c|}{91} &
  1 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{106} &
  \multicolumn{1}{c|}{140} &
  \multicolumn{1}{c|}{709} &
  \multicolumn{1}{c|}{134} &
  3 &
  \multicolumn{1}{c|}{99} &
  \multicolumn{1}{c|}{117} &
  \multicolumn{1}{c|}{502} &
  \multicolumn{1}{c|}{110} &
  4 &
  \multicolumn{1}{c|}{93} &
  \multicolumn{1}{c|}{76} &
  \multicolumn{1}{c|}{293} &
  \multicolumn{1}{c|}{69} &
  8 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# 3-Route\\ Breaks\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{134} &
  \multicolumn{1}{c|}{152} &
  \multicolumn{1}{c|}{628} &
  \multicolumn{1}{c|}{133} &
  6 &
  \multicolumn{1}{c|}{119} &
  \multicolumn{1}{c|}{114} &
  \multicolumn{1}{c|}{421} &
  \multicolumn{1}{c|}{102} &
  10 &
  \multicolumn{1}{c|}{82} &
  \multicolumn{1}{c|}{68} &
  \multicolumn{1}{c|}{183} &
  \multicolumn{1}{c|}{56} &
  10 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{0.62} &
  \multicolumn{1}{c|}{0.71} &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.75} &
  0.66 &
  \multicolumn{1}{c|}{0.67} &
  \multicolumn{1}{c|}{0.76} &
  \multicolumn{1}{c|}{0.76} &
  \multicolumn{1}{c|}{0.76} &
  0.67 &
  \multicolumn{1}{c|}{0.74} &
  \multicolumn{1}{c|}{0.79} &
  \multicolumn{1}{c|}{0.76} &
  \multicolumn{1}{c|}{0.76} &
  0.63 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{0.58} &
  \multicolumn{1}{c|}{0.69} &
  \multicolumn{1}{c|}{0.70} &
  \multicolumn{1}{c|}{0.73} &
  0.64 &
  \multicolumn{1}{c|}{0.63} &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.74} &
  0.59 &
  \multicolumn{1}{c|}{0.72} &
  \multicolumn{1}{c|}{0.75} &
  \multicolumn{1}{c|}{0.77} &
  \multicolumn{1}{c|}{0.73} &
  0.57 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{Fairness}} &
  \textbf{40} &
  \multicolumn{1}{c|}{0.53} &
  \multicolumn{1}{c|}{0.68} &
  \multicolumn{1}{c|}{0.66} &
  \multicolumn{1}{c|}{0.72} &
  0.59 &
  \multicolumn{1}{c|}{0.61} &
  \multicolumn{1}{c|}{0.71} &
  \multicolumn{1}{c|}{0.70} &
  \multicolumn{1}{c|}{0.71} &
  0.56 &
  \multicolumn{1}{c|}{0.70} &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.73} &
  \multicolumn{1}{c|}{0.74} &
  0.57 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{6} &
  5 &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{6} &
  4 &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{8} &
  \multicolumn{1}{c|}{6} &
  4 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  4 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  3 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  3 \\ \cline{3-18} 
\multicolumn{1}{|c|}{\multirow{-12}{*}{\textbf{40 m/s}}} &
  \multirow{-3}{*}{\textbf{$V_f$}} &
  \textbf{40} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{4} &
  4 &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{4} &
  2 &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{5} &
  2 \\ \hline

\Xhline{1pt}   
\end{tabular}

\end{adjustbox}
\end{table*}

==> Tables/table-3targets-50UAVs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\setlength{\tabcolsep}{3pt} % Default value: 6pt
\renewcommand{\arraystretch}{1.2} % Default value: 1
\begin{adjustbox}{width=\textwidth}
 
\begin{tabular}{|cc|c!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccccc!{\vrule width 1.5pt}ccccc|}

\hline
\multicolumn{2}{|c|}{} &
   &
  \multicolumn{5}{c|}{\textbf{Location={[}Case 7{]}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}Case5{]}}} &
  \multicolumn{5}{c|}{\textbf{Location={[}Case6{]}}} \\ \cline{4-18} 
\multicolumn{2}{|c|}{\multirow{-2}{*}{\textbf{50 UAVs}}} &
  \multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\% Node\\ Failure\end{tabular}}} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} &
  \multicolumn{1}{c|}{\textbf{TC}} &
  \multicolumn{1}{c|}{\textbf{Pipe}} &
  \multicolumn{1}{c|}{\textbf{AODV}} &
  \multicolumn{1}{c|}{\textbf{ConCov*}} &
  \textbf{Relay} \\ \hline
\Xhline{1pt}
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{99} &
  \multicolumn{1}{c|}{96} &
  \multicolumn{1}{c|}{88} &
  \multicolumn{1}{c|}{87} &
  100 &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{90} &
  \multicolumn{1}{c|}{78} &
  \multicolumn{1}{c|}{77} &
  100 &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{86} &
  \multicolumn{1}{c|}{71} &
  \multicolumn{1}{c|}{69} &
  100 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{98} &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{87} &
  \multicolumn{1}{c|}{81} &
  100 &
  \multicolumn{1}{c|}{91} &
  \multicolumn{1}{c|}{82} &
  \multicolumn{1}{c|}{72} &
  \multicolumn{1}{c|}{65} &
  100 &
  \multicolumn{1}{c|}{88} &
  \multicolumn{1}{c|}{75} &
  \multicolumn{1}{c|}{64} &
  \multicolumn{1}{c|}{57} &
  99 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Route\\ Up \%\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{96} &
  \multicolumn{1}{c|}{92} &
  \multicolumn{1}{c|}{84} &
  \multicolumn{1}{c|}{71} &
  100 &
  \multicolumn{1}{c|}{83} &
  \multicolumn{1}{c|}{75} &
  \multicolumn{1}{c|}{66} &
  \multicolumn{1}{c|}{51} &
  98 &
  \multicolumn{1}{c|}{75} &
  \multicolumn{1}{c|}{62} &
  \multicolumn{1}{c|}{54} &
  \multicolumn{1}{c|}{41} &
  98 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{26} &
  \multicolumn{1}{c|}{47} &
  \multicolumn{1}{c|}{546} &
  \multicolumn{1}{c|}{85} &
  0 &
  \multicolumn{1}{c|}{51} &
  \multicolumn{1}{c|}{86} &
  \multicolumn{1}{c|}{847} &
  \multicolumn{1}{c|}{123} &
  1 &
  \multicolumn{1}{c|}{71} &
  \multicolumn{1}{c|}{109} &
  \multicolumn{1}{c|}{1026} &
  \multicolumn{1}{c|}{151} &
  1 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{38} &
  \multicolumn{1}{c|}{65} &
  \multicolumn{1}{c|}{524} &
  \multicolumn{1}{c|}{93} &
  3 &
  \multicolumn{1}{c|}{79} &
  \multicolumn{1}{c|}{107} &
  \multicolumn{1}{c|}{751} &
  \multicolumn{1}{c|}{137} &
  5 &
  \multicolumn{1}{c|}{116} &
  \multicolumn{1}{c|}{141} &
  \multicolumn{1}{c|}{874} &
  \multicolumn{1}{c|}{166} &
  6 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Route\\ Breaks\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{57} &
  \multicolumn{1}{c|}{90} &
  \multicolumn{1}{c|}{489} &
  \multicolumn{1}{c|}{102} &
  5 &
  \multicolumn{1}{c|}{107} &
  \multicolumn{1}{c|}{134} &
  \multicolumn{1}{c|}{655} &
  \multicolumn{1}{c|}{134} &
  10 &
  \multicolumn{1}{c|}{157} &
  \multicolumn{1}{c|}{161} &
  \multicolumn{1}{c|}{711} &
  \multicolumn{1}{c|}{154} &
  13 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.86} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.84} &
  0.81 &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.84} &
  0.77 &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.84} &
  0.76 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{0.81} &
  \multicolumn{1}{c|}{0.83} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.82} &
  0.79 &
  \multicolumn{1}{c|}{0.81} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.82} &
  0.73 &
  \multicolumn{1}{c|}{0.81} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.82} &
  0.72 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{Fairness}} &
  \textbf{40} &
  \multicolumn{1}{c|}{0.76} &
  \multicolumn{1}{c|}{0.79} &
  \multicolumn{1}{c|}{0.80} &
  \multicolumn{1}{c|}{0.80} &
  0.74 &
  \multicolumn{1}{c|}{0.77} &
  \multicolumn{1}{c|}{0.82} &
  \multicolumn{1}{c|}{0.82} &
  \multicolumn{1}{c|}{0.80} &
  0.68 &
  \multicolumn{1}{c|}{0.77} &
  \multicolumn{1}{c|}{0.81} &
  \multicolumn{1}{c|}{0.81} &
  \multicolumn{1}{c|}{0.81} &
  0.65 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{5} &
  5 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  5 &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{7} &
  \multicolumn{1}{c|}{5} &
  4 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{10} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{5} &
  5 &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{5} &
  4 &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{6} &
  \multicolumn{1}{c|}{5} &
  3 \\ \cline{3-18} 
\multicolumn{1}{|c|}{\multirow{-12}{*}{\textbf{20 m/s}}} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Visitation\\ Frequency\end{tabular}}} &
  \textbf{30} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{4} &
  4 &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{4} &
  3 &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{5} &
  \multicolumn{1}{c|}{4} &
  2 \\ \hline
\Xhline{1pt}
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{98} &
  \multicolumn{1}{c|}{95} &
  \multicolumn{1}{c|}{80} &
  \multicolumn{1}{c|}{85} &
  100 &
  \multicolumn{1}{c|}{93} &
  \multicolumn{1}{c|}{87} &
  \multicolumn{1}{c|}{64} &
  \multicolumn{1}{c|}{72} &
  100 &
  \multicolumn{1}{c|}{92} &
  \multicolumn{1}{c|}{82} &
  \multicolumn{1}{c|}{56} &
  \multicolumn{1}{c|}{65} &
  100 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{98} &
  \multicolumn{1}{c|}{94} &
  \multicolumn{1}{c|}{79} &
  \multicolumn{1}{c|}{80} &
  100 &
  \multicolumn{1}{c|}{88} &
  \multicolumn{1}{c|}{79} &
  \multicolumn{1}{c|}{60} &
  \multicolumn{1}{c|}{62} &
  100 &
  \multicolumn{1}{c|}{84} &
  \multicolumn{1}{c|}{71} &
  \multicolumn{1}{c|}{51} &
  \multicolumn{1}{c|}{52} &
  99 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Route\\ Up \%\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{96} &
  \multicolumn{1}{c|}{89} &
  \multicolumn{1}{c|}{78} &
  \multicolumn{1}{c|}{72} &
  100 &
  \multicolumn{1}{c|}{79} &
  \multicolumn{1}{c|}{69} &
  \multicolumn{1}{c|}{55} &
  \multicolumn{1}{c|}{52} &
  99 &
  \multicolumn{1}{c|}{71} &
  \multicolumn{1}{c|}{56} &
  \multicolumn{1}{c|}{41} &
  \multicolumn{1}{c|}{36} &
  98 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{52} &
  \multicolumn{1}{c|}{98} &
  \multicolumn{1}{c|}{1025} &
  \multicolumn{1}{c|}{141} &
  1 &
  \multicolumn{1}{c|}{113} &
  \multicolumn{1}{c|}{169} &
  \multicolumn{1}{c|}{1520} &
  \multicolumn{1}{c|}{219} &
  1 &
  \multicolumn{1}{c|}{157} &
  \multicolumn{1}{c|}{229} &
  \multicolumn{1}{c|}{1799} &
  \multicolumn{1}{c|}{271} &
  1 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{77} &
  \multicolumn{1}{c|}{130} &
  \multicolumn{1}{c|}{997} &
  \multicolumn{1}{c|}{165} &
  3 &
  \multicolumn{1}{c|}{162} &
  \multicolumn{1}{c|}{212} &
  \multicolumn{1}{c|}{1345} &
  \multicolumn{1}{c|}{235} &
  5 &
  \multicolumn{1}{c|}{225} &
  \multicolumn{1}{c|}{293} &
  \multicolumn{1}{c|}{1536} &
  \multicolumn{1}{c|}{268} &
  8 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\# Route\\ Breaks\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{109} &
  \multicolumn{1}{c|}{172} &
  \multicolumn{1}{c|}{948} &
  \multicolumn{1}{c|}{177} &
  6 &
  \multicolumn{1}{c|}{207} &
  \multicolumn{1}{c|}{250} &
  \multicolumn{1}{c|}{1140} &
  \multicolumn{1}{c|}{226} &
  10 &
  \multicolumn{1}{c|}{283} &
  \multicolumn{1}{c|}{295} &
  \multicolumn{1}{c|}{1174} &
  \multicolumn{1}{c|}{240} &
  14 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.90} &
  \multicolumn{1}{c|}{0.90} &
  \multicolumn{1}{c|}{0.89} &
  0.86 &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.91} &
  \multicolumn{1}{c|}{0.91} &
  \multicolumn{1}{c|}{0.89} &
  0.84 &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.92} &
  \multicolumn{1}{c|}{0.89} &
  0.83 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.87} &
  \multicolumn{1}{c|}{0.88} &
  0.82 &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.88} &
  \multicolumn{1}{c|}{0.88} &
  0.81 &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.89} &
  \multicolumn{1}{c|}{0.88} &
  0.76 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
  \multirow{-3}{*}{\textbf{Fairness}} &
  \textbf{40} &
  \multicolumn{1}{c|}{0.78} &
  \multicolumn{1}{c|}{0.84} &
  \multicolumn{1}{c|}{0.83} &
  \multicolumn{1}{c|}{0.87} &
  0.80 &
  \multicolumn{1}{c|}{0.81} &
  \multicolumn{1}{c|}{0.85} &
  \multicolumn{1}{c|}{0.86} &
  \multicolumn{1}{c|}{0.86} &
  0.76 &
  \multicolumn{1}{c|}{0.81} &
  \multicolumn{1}{c|}{0.86} &
  \multicolumn{1}{c|}{0.86} &
  \multicolumn{1}{c|}{0.86} &
  0.73 \\ \cline{2-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{0} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{10} &
  10 &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{10} &
  9 &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{13} &
  \multicolumn{1}{c|}{10} &
  9 \\ \cline{3-18} 
\multicolumn{1}{|c|}{} &
   &
  \textbf{20} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{9} &
  9 &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{9} &
  7 &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{12} &
  \multicolumn{1}{c|}{9} &
  6 \\ \cline{3-18} 
\multicolumn{1}{|c|}{\multirow{-12}{*}{\textbf{40 m/s}}} &
  \multirow{-3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Visitation\\ Frequency\end{tabular}}} &
  \textbf{40} &
  \multicolumn{1}{c|}{10} &
  \multicolumn{1}{c|}{10} &
  \multicolumn{1}{c|}{10} &
  \multicolumn{1}{c|}{8} &
  8 &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{10} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{8} &
  5 &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{11} &
  \multicolumn{1}{c|}{10} &
  \multicolumn{1}{c|}{8} &
  5 \\ \hline

\Xhline{1pt}   
\end{tabular}

\end{adjustbox}
\end{table*}
